Improved Policy Evaluation for Randomized Trials of Algorithmic Resource Allocation

We consider the task of evaluating policies of algorithmic resource allocation through randomized controlled trials (RCTs). Such policies are tasked with optimizing the utilization of limited intervention resources, with the goal of maximizing the benefits derived. Evaluation of such allocation policies through RCTs proves difficult, notwithstanding the scale of the trial, because the individuals' outcomes are inextricably interlinked through resource constraints controlling the policy decisions. Our key contribution is to present a new estimator leveraging our proposed novel concept, that involves retrospective reshuffling of participants across experimental arms at the end of an RCT. We identify conditions under which such reassignments are permissible and can be leveraged to construct counterfactual trials, whose outcomes can be accurately ascertained, for free. We prove theoretically that such an estimator is more accurate than common estimators based on sample means -- we show that it returns an unbiased estimate and simultaneously reduces variance. We demonstrate the value of our approach through empirical experiments on synthetic, semi-synthetic as well as real case study data and show improved estimation accuracy across the board.

==> intro-aditya-v0.tex <==
% As a result, even if a large number of participants are involved in the trial, they only amount to a single instance of the trial, yielding one random sample of the policy performance --- a far cry from the large number of independent samples desired. This necessitates methods to build better estimators of such resource allocation policies' performance through clinical trials.
% Popular causal inference methods such as linear regression modeling \citep{}, t-tests \citep{} or ANNOVA \citep{} are inadequate to generate valid inference on such adaptively collected data. 
% In fact, such a clinical trial yields only a single sample of the performance on a single instance of a test experimental cohort, necessitating methods to build better estimators of the performance of such resource allocation algorithms through clinical trials.  
The main roadblock is that the goal is to evaluate the allocation quality of interventions and not the effect of interventions themselves. We argue that, as a consequence, the noise stemming from randomized instantiation of the experimental arms may still remain substantial, notwithstanding the large participant strength, $N$. 
Intuitively, there may be a large chunk of the cohort that may never receive an intervention, no matter the choice of policy employed in the experimental arm. Similarly, no matter the policy, many agents in the cohort may always get earmarked for intervention delivery by all test policies. The outcomes of such agents are indifferent to the evaluation group they belong to, and thus carry no signal of the policies' performance. A larger proportion of such participants may overshadow the outcomes from signal-carrying participants, making it hard to evaluate policy performance or achieve statistical significance through such trials.

As a fix, our central idea is to identify agents in the trial whose intervention decisions (and consequently, outcomes) remain unaffected by the experimental group they are assigned to. In other words, we identify a subset of agents $\mathcal{A}$ in the trial, satisfying the following property: 
\textit{For any two agents $a_i, a_j~ \in \mathcal{A}$ assigned to arms $i, j ~\in \{1,\dots m\}$ respectively in the trial, if we were to run a hypothetical trial with their arm assignments swapped (i.e. by assigning $a_i$ to arm $j$ and $a_j$ to arm $i$), the new intervention decisions received remain unaltered from the original trial and the new trial still looks identical from the perspectives of $a_i$ and $a_j$.}
% where an agent $a \in \mathcal{A}$ is assigned to an experimental arm $a_i, \dots a_m$ such that $a_i$ belongs to experimental arm $i$ in the trial. Furthermore, this set is such that, if we ran a hypothetical experiment, with any other counterfactual assignment of $[a_m]$ agents to $[m]$ experimental arms, nothing about the intervention decisions received by any of the participants in the trial would have changed from the original experiment.
In this special circumstance, we argue that for such a counterfactual trial with reassigned groups, with all inputs to all individuals remaining identical, the individual outcomes observed for all agents would also remain unchanged. This essentially allows us to consider several additional counterfactual instances of random assignments (and equivalently, counterfactual clinical trials) and uncover their counterfactual experimental outcomes for free. 

% \hl{May be useful to describe the toy example and the intuition here instead of experiments section and only defer details of results to that section.}

Our key contribution in this paper is to first propose this novel concept of retrospectively permuting experimental cohorts in clinical trials for improved performance estimation of resource allocation algorithms. Second, we show theoretically that our estimator is unbiased and reduces the sample variance --- proving that our approach yields a more accurate estimate than simpler methods. Finally, we back our approach through empirical experiments on three domains --- leveraging synthetic, semi-real and real-world case study data --- and show improved estimation across the board. 

% Intuitively, the key roadblock is that the number of interventions delivered in such settings is typically a much smaller fraction of the experimental arm size (motivating the need for a clever intervention allocation algorithm in the first place). 

% In following sections, we formalize the problem statement, present the cohort permutation methodology and algorithm and demonstrate results on synthetic and real-world clinical trials. \hl{TODO: Solidify Contributions summary paragraph}


==> intro-bryan-v1.tex <==
In a standard RCT, the aim is to evaluate the treatment effect (e.g., of receiving a resource) for the average participant. As the outcomes of all participants are independent, analysts can simply compare outcomes in the treatment versus control groups. However, trials of resource allocation policies aim to evaluate the \textit{group} outcome of a set of individuals to whom the policy is applied (some of whom receive the resource, and some who do not). Even when the number of individuals in the trial is large by the standards of a normal RCT, this means that randomized trials of allocation policies can suffer from high variance, leading to noisy and potentially erroneous estimates of the treatment effect. This high variance arises from two sources. First, the outcomes of agents within an given arm are correlated because allocation policies typically consider all agents \textit{jointly} in making an allocation decision (e.g., to respect budget constraints on the total number of agents who may receive an intervention). Second, allocation policies are often used in settings where the resource is scarce, meaning that many individuals do not receive an allocation. These individuals are not truly impacted by the policy, but their presence generates additional variance in the average outcome of the group due to noise which is independent of the resource allocation. 

To our knowledge, no prior work confronts the challenge of RCTs for resource allocation policies, a critical gap given the increasing use of algorithmic policies in socially important domains. An intuitive first attempt would be to overcome the increased variance of such trials by sharing information across arms. For example, we could average out fluctuations in the outcomes of individuals who do not receive an allocation by pooling together such individuals across all of the policies that were tested. Unfortunately, such naive estimators are biased because the distribution of \textit{which} individuals receive a resource (or not) is different across the trial arms -- indeed, assessing the comparative efficacy of these distributions is exactly the point of the trial. A more sophisticated strategy would be to exploit overlap between the policies via inverse propensity weighting estimators which reweight participants in one arm to match the actions a different policy would have taken. However, such estimators are themselves subject to notoriously high variance. Moreoever, as we discuss in detail below, propensity scores are impossible to calculate in the case of sequential interventions, where unseen potential outcomes prevent us from evaluating individual-level propensities for a different policy.

Our key contribution is a novel estimator for the treatment effect of resource allocation policies which exploits overlap between arms in a principled manner, is guaranteed to reduce variance, and is applicable to either single-stage or sequential settings. The main idea is to find a subset of individuals with the following property: if we ran a hypothetical trial where the arm assignments of these individuals were swapped, the allocations made for all individuals are not changed. Our estimator takes a set of individuals with this property and averages the outcomes of all such hypothetical trials (which are observable because no allocation decisions were altered from the original trial). We make the following contributions: (1) we propose this novel estimator and prove that it produces an unbiased estimate of the treatment effect with a guaranteed reduction in variance compared to the standard estimator, implying that it has strictly smaller average error; (2) we show how this estimator can be implemented in a computationally efficient manner for a class of policies encompassing those most commonly used in real-world allocation decisions (3) we conduct experiments on three domains -- leveraging synthetic, semi-synthetic, and real-world case study data -- and demonstrate that our estimator results in substantially reduced error (up to X\%) compared to baselines. 


==> old-sec4.2.tex <==
The key idea behind our estimator is to identify hypothetical trials with counterfactual experimental group assignments, whose outcomes can be exactly determined from the given outcomes from the original trial. We leverage the fact that the stochasticity in state transition (and equivalently, the outcome) of an individual is solely tied to its current state $s$ and the intervention decision received $a$ but is indifferent, and infact, oblivious to the policy $\pi$ responsible for choosing $a$. Consider a thought experiment in which the original trial was run, but with a different, hypothetical group assignment, constructed by interchanging assignments of two distinct individuals $i$ and $j$ belonging to distinct policy groups $\pi_i$ and $\pi_j$ in the original trial. 
In this thought experiment, if both $i$ and $j$ at all timesteps, were to receive allocations from their respective new policies that are identical to the actual allocations that they received in the actual trial, then, to all participants in the trial, the hypothetical trial would be indistinguishable from the actual. In other words, the state trajectories of $i$ and $j$ embody valid samples of the state trajectories in both, the actual as well as the hypothetical trial.  
% then the swapping would have had no bearing on their state transitions (and consequently outcomes).
% trial in which group assignments of two individuals $i$ and $j$ belonging to policy groups $\pi_i$ and $\pi_j$ in the original trial, are interchanged. 
% If both $i$ and $j$, under their respective new policies see the same allocations as the original trial, for all timesteps, then the swapping would have had no bearing on their state transitions (and consequently outcomes). 
% In other words, the ensuing state trajectories of $i$ and $j$ in the counterfactual trial would remain exactly as originally observed. 
% Generalizing this idea, if an individual's group assignment in the trial were to be swapped with another individual in a different arm employing a policy $\pi^\dag$, such that for all individuals, the new intervention decisions $a^\dag (t) \coloneqq \pi^\dag(\textbf{X}^\dag_o, \textbf{s}^\dag_{0: t-1}, \textbf{a}^\dag_{1:t-1})$, were identical to $a(t)$, $\forall t \in [T]$, then the individual's state trajectory $s^\dag$, no longer remains an unseen counterfactual, as it would be identical to the original trajectory $s$. 
% Generalizing this idea, if a subset of individuals' group assignments in the trial were permuted to arrive at a new assignment $\mathfrak{C}^\dag$, such that for all individuals, the resultant new actions $a^\dag (t)$ remain identical to $a(t)~\forall t \in [T]$, then the individual's state trajectory $s^\dag(t)$ no longer remains an unseen counterfactual but can be inferred to be identical to the original trajectory $s(t)$.
Generalizing this idea, if a subset of individuals' group assignments in the trial were permuted to arrive at a new assignment $\mathfrak{C}^\dag$, such that for all individuals, the resultant new actions $a^\dag (t)$ generated using the original state trajectory $s(t)$ as input, remain identical to the original, $a(t)~\forall t \in [T]$, then we argue that the original state trajectory is a valid sample of the individuals' unseen counterfactual state trajectory $s^\dag(t)$.
We exploit this concept to retrospectively check for all such possible reassignments, that would lead to the same sequence of decisions received. The implication is that this allows us to uncover and aggregate outcomes from several such additional `observable counterfactual assignments' (defined below) in estimating the performance of a given test policy. Algorithm~\ref{alg:algorithm-shuffling-general} outlines the general idea for a general $M$-arm setting. Later, in Algorithm~\ref{alg:shuffling-index-index} we present an efficient algorithm crafted for handling index-based policies. 

